An Entity-Driven Framework for Abstractive Summarization

Abstractive summarization systems aim to produce more coherent and concise summaries than their extractive counterparts. Popular neural models have achieved impressive results for single-document summarization, yet their outputs are often incoherent and unfaithful to the input. In this paper, we introduce SENECA, a novel System for ENtity-drivEn Coherent Abstractive summarization framework that leverages entity information to generate informative and coherent abstracts. Our framework takes a two-step approach: (1) an entity-aware content selection module first identifies salient sentences from the input, then (2) an abstract generation module conducts cross-sentence information compression and abstraction to generate the final summary, which is trained with rewards to promote coherence, conciseness, and clarity. The two components are further connected using reinforcement learning. Automatic evaluation shows that our model significantly outperforms previous state-of-the-art on ROUGE and our proposed coherence measures on New York Times and CNN/Daily Mail datasets. Human judges further rate our system summaries as more informative and coherent than those by popular summarization models.

==> humaneval.tex <==
We further conduct human evaluation to analyse the informativeness and readability of the summaries generated by our models. For this, we randomly select 30 input articles from NYT dataset and ask three proficient English speakers to rate summaries generated by \textsc{PointGen+cov}, \textsc{ML+RL}(\newcite{paulus2017deep})~\footnote{Since, we do not have model output from the authors, we use ones generated from our implementation for the same (Rouge Metrics for this are R1:46.61,R2:29.76 and RL:43.46}, \textsc{Ent} and \textsc{EntCoh}, along with the gold-standard \textsc{Human} written summaries. Each rater reads the input article and rates the summaries against each other on a Likert scale of 1 (worst) to 5 (best) on the following three aspects: \textbf{informativeness}--whether summary covers all the salient points from the input article; \textbf{grammaticality}--whether summary is grammatically correct and \textbf{coherence}--whether summary presents information in systematic order. Ties between different system outputs were allowed but discouraged (See Supplementary for additional details). 
%  \textbf{entity usage}--whether discourse entities are used appropriately.
\begin{table}[h]
\centering
\fontsize{9}{11}\selectfont
 \setlength{\tabcolsep}{0.7mm}
\begin{tabular}{lccc}
\toprule
& {\bf Inf.} & {\bf Gram.} & {\bf Coh.} \\\midrule
     \textsc{Human} & 4.58 & 4.42 & 4.16    \\ \hdashline
    \textsc{PointGen+cov} & 3.63 & \textbf{4.47}  & 3.89    \\  
     \textsc{DeepReinforce}  & 3.63 & 3.21 & 3.16    \\ 
     \textsc{SENECA} & 4.26 & 4.11 & 4.05  \\
    \textsc{SENECA} + $R_{\rm Coh}$ & \textbf{4.32$^{\ast}$} & 4.10 & \textbf{4.11$^{\ast}$}   \\ \bottomrule
    \end{tabular}
\caption{%\fontsize{10}{12}\selectfont  
Human evaluation on informativeness (Inf.), grammaticality (Gram.) and coherence (Coh.). The best results among automatic systems are highlighted in bold, with statistical significance marked with $\ast$ (approximation randomization test, $p<0.0005$). The Krippendorf's $\alpha$ for three aspects are $0.46$, $0.64$, $0.48$, respectively.}
  \label{tab:human-eval}
\end{table}
Table ~\ref{tab:human-eval} shows that our model \textsc{EntCoh} ranks significantly higher on informativeness as well as coherence, reinforcing our automatic evaluation of the summaries on ROUGE and other coherence related metrics. Surprising, \textsc{EntCoh} ranks higher on informativeness even when compared to \textsc{Ent}, which reports higher on Rouge (refer to Table ~\ref{tab:nyt-rouge}). While doing manual inspection, we find that \textsc{Ent} model often generates summaries with second or third sentences missing the subject, which \textsc{EntCoh} corrects. For instance, compared to \textsc{Ent}'s output \textit{``vermont supreme court rejects host of arguments from isabella's biological mother, lisa miller. should be denied parental rights.''}, \textsc{EntCoh} generates \textit{``vermont supreme court rejects host of arguments from isabella's biological mother, lisa miller. her former lesbian partner, janet jenkins, should be denied parental rights.''}  Although not significantly, \textsc{PointGen+cov} ranks higher on grammaticality than \textsc{EntCoh}. We believe this is due to the fact that \textsc{Entcoh} learns to merge sentences from input article making grammatical errors in the process. 
% Table ~\ref{tab:human-eval} shows that our model \textsc{EntCoh} ranks significantly higher on informativeness as well as coherence, reinforcing our automatic evaluation of the summaries on ROUGE and other coherence related metrics. Surprising, \textsc{EntCoh} ranks higher on informativeness even when compared to \textsc{Ent}, which reports higher on Rouge (refer to Table ~\ref{tab:nyt-rouge}). While doing manual inspection, we find that \textsc{Ent} model often generates summaries with second or third sentences missing the subject, which \textsc{EntCoh} corrects. For instance, compared to \textsc{Ent}'s output \textit{``vermont supreme court rejects host of arguments from isabella's biological mother, lisa miller. should be denied parental rights.''}, \textsc{EntCoh} generates \textit{``vermont supreme court rejects host of arguments from isabella's biological mother, lisa miller. her former lesbian partner, janet jenkins, should be denied parental rights.''}  Although not significantly, \textsc{PointGen+cov} ranks higher on grammaticality than \textsc{EntCoh}. We believe this is due to the fact that \textsc{Entcoh} learns to merge sentences from input article making grammatical errors in the process. 


==> intro_v1.tex <==
\section{Introduction}
% \begin{comment}
% paragraph 1 -> types of summarization : extractive and abstractive -> list all the SOTAs.
% paragraph 2 -> what they have and what they loose - entity aware and coherence. What we introduce.
% paragraph 3 -> current models end to end approach flaw
% paragraph 4 -> coherence only for extractive summarization
% paragraph 6 -> contribution 1: Summarization Pipeline
% paragraph 7 -> RL rewards
% paragraph 8 -> Coherence evaluation suite
% paragraph 9 -> Results & layout
% \end{comment}
\begin{comment}
End to end abstractive summarization succeeds in blah blah. 
\end{comment}





Automatic text summarization is the task of compressing a long document into a short yet comprehensive excerpt, that retains the salient information from the original text. While extractive summaries can be generated by selecting these salient parts of the source document~\cite{zhou2018neural}, abstractive summarization additionally requires the ability to rephrase and restructure sentences to compose a coherent and concise summary~\cite{gehrmann-etal-2018-bottom,paulus2017deep,see-etal-2017-get}. 

In past, neural abstractive summarization models have combined extractive and abstractive techniques using approaches such as pointer networks~\cite{} and reinforcement learning~\cite{} to generate fluent asbtractive summaries. However, these end-to-end approaches tend to being slow and have to compromise on the length of input article to be encoded, compared to fully extractive models. 

Humans tend to break the summarization task into two steps. First, they scan the whole article to extract the salient parts of the document and then, use paraphrasing to compress these parts into a concise summary~\cite{}. In line with this observation, recent works have adopted a hybrid approach, where the two tasks, content selection and abstraction, are conveniently separated from each other. This not only helps the model to get better content coverage, but also helps reduce redundancy issues often encountered during abstraction~\cite{}.

While recent works employing the multi-step training have shown promising improvement over the informativeness aspect of the generated summaries, semantic understanding of salient entities and their relations in a document still largely remains unexplored. Discourse entities and their relations are not only important in terms of content selection but can also guide the model to generate structurally more coherent text. \newcite{wu2018learning} proposed a neural coherence model that captures cross-sentence coherence patterns and incorporated its output as a reward for their reinforcement learning based neural extractive summarization model to generate coherent extractive summaries. However, there has been little research on producing coherent abstracitve summaries. %(except for : Paulus using rouge-l as reward) 

To address aforementioned concerns, building upon the ~\newcite{chen-bansal-2018-fast} and ~\newcite{paulus2017deep}, we present hybrid summarization pipeline. It consists of an extractor trained with discourse entity supervision, that learns to select salient sentences from the whole input article and an abstractor explicitly guided by coherence based reinforcement learning rewards, that learns to generate coherent abstract summaries. The extractor and abstractor are finally jointly trained using Rouge-1 as reinforcement learning reward to produce the final summary.  

We evaluate our summarization pipeline on CNNDM and NYT dataset and achieve state of art results on both? datasets. We further employ automatic coherence evaluation, comparing the state-of-art model generated summaries against ours on several dimensions of coherence such as structural coherence, use of discourse connectors, referential pronoun clarity as well as discourse entity repetition. 

% Once model results are finalized - compare and include SOTA model summaries with ours on different aspects of content coverage as well as coherence.

Contributions of our summarized here. 



% \begin{table*}[ht!]
% \fontsize{9}{11}\selectfont
% \setlength{\tabcolsep}{0.8mm}{
% \begin{tabular}{p{\textwidth}}
% \toprule
% \textbf{Gold-Standard summary} \\
%  \\ \hline
% \textbf{\textsc{PGC} generated summary} \\
%  \\ \hline
% \textbf{\textsc{FastRL} generated summary} \\
%  \\ \hline
% \textbf{\textsc{Our Best Model} generated summary} \\ \hline
% \end{tabular}
% }
% \caption{Gold-standard and system generated summaries for New York Times dataset. Place holder table for now. }
% \vspace{-17pt}
% \label{tbl:samples}
% \end{table*}  
